The Rational Agent Benchmark for Data Visualization

Understanding how helpful a visualization is from experimental results is difficult because the observed performance is confounded with aspects of the study design, such as how useful the information that is visualized is for the task. We develop a rational agent framework for designing and interpreting visualization experiments. Our framework conceives two experiments with the same setup: one with behavioral agents (human subjects), and the other one with a hypothetical rational agent. A visualization is evaluated by comparing the expected performance of behavioral agents to that of a rational agent under different assumptions. Using recent visualization decision studies from the literature, we demonstrate how the framework can be used to pre-experimentally evaluate the experiment design by bounding the expected improvement in performance from having access to visualizations, and post-experimentally to deconfound errors of information extraction from errors of optimization, among other analyses.

==> 02b-example.tex <==


\subsection{Example: Pre-experimental Analysis for Weather Forecast}


\iffalse



%o\jessica{maybe a figure or table presentation of decision problem is better?}

The data generating process is as follows.  The daily low temperature
is generated from Gaussian distribution $N(\mu, \sigma^2)$ with a
deterministic mean $\mu=5^\circ C$ and standard deviation
$\sigma$. The standard deviation $\sigma$ is uniformly drawn from
$\{2, 3, 4, 5\}$.  For visualizations that depict uncertainty (CI,
gradient, HOPs), the signal $\signal$ is $(\mu,\sigma)$; for the visualization of the
mean, the signal $\signal$ is deterministically $\mu$. Since the visualizations are informationally inequivalent, we apply our general framework in \Cref{sec:general-information-asymmetry}. 

The payoff relevant state
$\state$ is from state space $\statespace = \{0 = \text{not freezing},
1 = \text{freezing}\}$.  The joint distribution $\joint \in \distover{\signalspace \times \statespace}$ on signal and state
for the three non-trivial visualization types is:

\begin{center}
\small
\begin{tabular}{l|cccc}
\hline
             & $\sigma = 2$ & $\sigma = 3$ & $\sigma = 4$ & $\sigma = 5$ \\
  \hline
  $\state = 0$  & $0.24845$ & $0.23805$ & $0.2236$ & $0.2103$ \\
  $\state = 1$  & $0.00155$ & $0.01195$ & $0.0264$ & $0.0397$ \\
  \hline
\end{tabular}
\normalsize
\end{center}

The rational agent calculates her prior and posterior distributions as
follows.  Note that a distribution $\dist$ on a binary state space
$\statespace = \{0,1\}$ can be fully described by the probability that
the binary state is $\state = 1$ (freezing).  From
\cref{eq:prior} we have \Yifan{the prior probability of freezing 
\begin{equation}
    p = \sum_\sigma \Pr[\state = 1 , \sigma]=0.00155+0.01195+0.0264+0.0397=0.0796,
\end{equation}
and the posterior probabilities after knowing $\sigma$ as given in \Cref{tab:example-notation}. Here we take $\sigma = 2$ as an example:
\begin{equation}
    \Pr[\state=1 | \sigma = 2] = \Pr_{ x\sim N(5, 2^2)}[x\leq 0]=0.0062.
\end{equation}
}%$\prior = 0.08$; from \cref{eq:posterior} we
%have posteriors as given in \Cref{tab:example-notation}.


The decision-maker must decide whether to salt the parking lot or not,
i.e., by selecting action $\action$ from action space $\actionspace =
\{0=\text{no salt}; 1=\text{salt}\}$.  Given the state space
$\statespace = \{0=\text{not freezing};1=\text{freezing}\}$ the
experimenter endows the following payoff function as a scoring rule:

\begin{equation}
    \score(\action, \state)=\left\{\begin{array}{ccc}
    0 & \text{if }a = 0, \state= 0
      & \textit{no salt, not freezing } \\
     -100    & \text{if }\action=0, \state=1
     & \textit{no salt, freezing}\\
    -10      & \text{if }\action=1, \state= 0
    & \textit{salt,  not freezing}\\
    0    &  \text{if } \action=1, \state=1
    & \textit{salt, freezing}
    \end{array}\right.
    \label{eq:salting}
\end{equation}
\fi



We perform our pre-experimental analysis on the hypothetical weather forecast experiment in \Cref{sec:salting-decision}. Since the visualizations are informationally inequivalent, we apply our general framework in \Cref{sec:general-information-asymmetry}. 

The rational agent calculates her prior and posterior distributions as
follows.  Note that a distribution $\dist$ on a binary state space
$\statespace = \{0,1\}$ can be fully described by the probability that
the binary state is $\state = 1$ (freezing).  From
\cref{eq:prior} we have the prior probability of freezing 
\begin{equation}
    p = \sum\nolimits_\sigma \Pr[\state = 1 , \sigma]=0.00155+0.01195+0.0264+0.0397=0.0796,
\end{equation}
and the posterior probabilities are $\Pr[\state=1|\sigma]=0.62\%, 4.78\%, 10.56\%, 15.87\%$, relatively for $\sigma=2, 3, 4, 5$, as given in \Cref{tab:example-notation}. Here we take $\sigma = 2$ as an example:
\begin{equation}
    \Pr[\state=1 | \sigma = 2] = \Pr_{ x\sim N(5, 2^2)}[x\leq 0]=0.0062.
\end{equation}

\Cref{fig:weather_payoff} depicts the expected score of the agent for both no-salt and salt actions as a function of his belief
$\dist$, as specified in \Cref{eq:salting}.  Notice that if the belief is certainty $\dist \in \{0,1\}$
then the payoff is given explicitly by the scoring rule.  For an
uncertain belief $\dist \in (0,1)$ the payoff is given by linearly
interpolating between the certain beliefs, i.e., the payoff is the
expected value of the action over the belief.  Lines correspond to the no-salt and salt action.  The optimal
action for each posterior belief -- i.e., the action taken by the
rational agent -- can be read off as well.  For each
signal, we find its posterior on the horizontal axis, and evaluate
which of the two actions give a higher payoff and take that one.  From
this analysis it is clear that the no-salt action $\action = 0$ is
taken on the lower two signals $\{2,3\}$ and the salt action
$\action=1$ is taken on the higher two signals $\{4,5\}$. The payoff
lines cross at $\dist = 0.9$ where the decision-maker is indifferent
between no-salt and salt actions.

The rational agent framework gives the following quantities:
\begin{description}
\item[rational baseline:] $\rprior = -7.96$.  

  The prior $\prior = 0.08$ is optimized at no-salt and gives an expected payoff of $-7.96$. The calculation is as following:
\begin{align*}
    \rprior &= \Pr[\state=0]\cdot\score(\action = 0, \state=0) + \Pr[\state=1]\cdot\score(\action = 0, \state=1)\\
    &= (1-0.0796)\times 0 + 0.0796\times (-100)=-7.96
\end{align*}
  

\item[visualization optimal:] 
  $\rpos^{\text{CI}}=\rpos^{\text{gradient}}=\rpos^{\text{HOPs}}=-5.69$; $\rpos^{\text{mean}}=-7.96$.
  
  In CI, gradient, and HOPs, each signal arises with probability $1/4$ and the average of the optimal actions under the induced posteriors (read off \Cref{fig:weather_payoff}) gives $\rpos = -5.69$.  For the visualization of the mean, the rational agent has only the prior information and obtains $\rpos^{\text{mean}} = \rprior = -7.59$.

  The calculation of $\rpos$ for CI, gradient, and HOPs is the following:
  \begin{align*}
      \rpos^{\text{CI}} &= \sum\nolimits_{\sigma, \state}\Pr[\sigma, \state]\cdot \score(\mathbf{1}_{\sigma\in\{4, 5\}}, \state)\\
      &= 0.24845\times 0 + 0.00155\times (-100)+0.23805\times 0 + 0.01195\times (-100)\\
      &\quad + 0.2236\times (-10) + 0.0264\times 0 + 0.2103\times (-10) + 0.0397\times 0\\
      &= -5.69
  \end{align*}
 \item[rational benchmark:] $\rperfect = \max_v \rscore^v = -5.69$, the best achievable across visualizations. 
\item[value of information:]  $\infoval = \rperfect - \rprior = 2.27$.%$\infoval^{\text{CI}}=\infoval^{\text{gradient}} = \infoval^{\text{HOPs}} = 2.27$; $\infoval^{\text{mean}} = 0$

  \end{description}
    % \jessica{Once the experimenter conducts the experiment, the behavioral scores can be used to assess differentiation loss from each visualization}
     
   %  \jessica{Yifan - fix. spell out the reasoning for making the scoring rule better given that you see the negative payoffs}
     %If the experimenter runs this decision task, she faces a minimum wage constraint. %\jessica{this minimum wage thing comes out of nowhere; what is the general approach that is being applied here? is it explained above?}
 %    The experimenter can assign each agent  $100$  decision questions with  $\sigma$ drawn uniformly from $[0, 5]$.  With high probability, the simulated payoff with not salting is above $-6$. The experimenter can set the payoff rule so that the participant gets a guaranteed payment of minimum wage (e.g.\ $\$1$) whenever the average simulated payoff is above $-6$, while the conversion rate for bonus is $\$1$ per $1$ simulated payoff above $-6$. Under such a payment scheme, the rational agent has an incentive of $\$0.99$ to finish the tasks. Comparing to the expected highest payment of $3.26$ and a guaranteed payment of $\$2.27$ by playing the same action, the ratio of incentive to guaranteed payment is good enough. %\jessica{need to spell out why}
 %\end{itemize}

 Suppose the experimenter sets the conversion rule $f(\reward) = \$1+\$0.01\reward$ from score $\reward$ to real dollars as follows: an agent gains a fixed $\$1$ for completing each trial,  plus a $\$0.01$ in real dollars for each point earned in scoring rule space.  The conversion rule is set such that an agent is guaranteed to obtain a positive payment. We calculate the expected real payments to a rational agent in  \Cref{tab:forecast-incentive}. If the goal is to incentivize an agent to consult the visualization, the incentive is badly designed because it is a very small fraction of the amount expected without looking at the visualizations. 
 
 
\begin{table}[htbp]
\small
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
     $f(\rprior)$ & $f(\rpos)$ &  $\Delta_f$ & $\Delta_f / f(\rprior)$\\
     \hline
     $\$0.920$ & $\$0.943$ & $\$0.023$ & $2.5\%$\\
    \hline
    \end{tabular}
    \caption{$f(\rprior)$ shows the expected payment to a rational agent, $f(\rpos)$ shows the expected payment to a rational agent who reads the visualization, while $\Delta_f=f(\rpos)-f(\rprior)$ is the incentive to consult the visualization.}
    \normalsize
    \vspace{-2mm}
    \label{tab:forecast-incentive}
\end{table}

The infomation loss can also be calculated pre-experimentally.
\begin{description}
    \item[information loss]  CI, gradient, and HOPs: $(\rperfect-\rpos)/\infoval = 0$. Mean: $(\rperfect - \rpos^{\text{mean}})/\infoval = 100\%$. 
\end{description}

From this pre-experiment analysis, the experimenter should also expect the mean visualization to behave badly in payoff compared to the interval, because the mean is not informative for the decision task. If the researcher believes that showing only a mean is well motivated to study (e.g., because many weather forecasts report only an expected temperature), this may be a valid comparison. However, it should not be considered surprising when behavioral agents do poorly. 

%For the other conditions, the value of information ($\Delta = 2.27$) is slightly less than half the expected baseline score,
%providing a reasonable incentive to consult the visualizations.
%If the data-generating model were designed differently, such that the optimal decision relies heavily on the mean, the visualization of mean would be comparable to other visualizations. This highlights the dependence of results on the DGM, and the value of benchmarks that account for the experiment design. \jessica{not sure about prev two sentences}

   %  After conducting the experiment, the researcher can calculate the behavioral value of information for each visualization type, and express these scores as a ratio of the value of information to get a concise summary of what proportion of the attainable information gain participants were able to achieve. By calibrating the behavioral scores for each visualization type to calculate differentiation loss and decision loss, the researcher could present results that distinguish the extent to which each visualization contributed to failures of information extraction versus difficulty translating the information to a decision.
  

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{vis2023/figure/weather_payoff.pdf}
    \vspace{-3mm}
    \caption{Score $\score(\action,\dist)$ as a function of belief $\dist \in [0,1]$ as probability of freezing.}
    \vspace{-3mm}
    \label{fig:weather_payoff}
\end{figure}

